Exploring Chemical Homogeneity in Dwarf Galaxies: A VLT-MUSE study of JKB 18

Deciphering the distribution of metals throughout galaxies is fundamental in our understanding of galaxy evolution. Nearby, low-metallicity, star-forming dwarf galaxies in particular can offer detailed insight into the metal-dependent processes that may have occurred within galaxies in the early Universe. Here we present VLT/MUSE observations of one such system, JKB 18, a blue diffuse dwarf galaxy with a metallicity of only 12+log(O/H)=7.6$\pm$0.2 (~0.08 Zsol). Using high spatial-resolution integral field spectroscopy of the entire system, we calculate chemical abundances for individual HII regions using the direct method and derive oxygen abundance maps using strong-line metallicity diagnostics. With large-scale dispersions in O/H, N/H and N/O of ~0.5-0.6 dex and regions harbouring chemical abundances outside this 1$\sigma$ distribution, we deem JKB 18 to be chemically inhomogeneous. We explore this finding in the context of other chemically inhomogeneous dwarf galaxies and conclude that neither the accretion of metal-poor gas, short mixing timescales, or self-enrichment from Wolf-Rayet stars are accountable. Using a galaxy-scale, multi-phase, hydrodynamical simulation of a low-mass dwarf galaxy, we find that chemical inhomogeneities of this level may be attributable to the removal of gas via supernovae and the specific timing of the observations with respect to star-formation activity. This study not only draws attention to the fact that dwarf galaxies can be chemically inhomogeneous, but also that the methods used in the assessment of this characteristic can be subject to bias.

==> All_fluxes_combined0_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~0} & \multicolumn{2}{c|}{\hii\ Reg~1 }& \multicolumn{2}{c|}{\hii\ Reg~2} & \multicolumn{2}{c|}{\hii\ Reg~3} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
    3.71$\pm$   0.29 &     3.77$\pm$   0.29 & 
    3.15$\pm$   0.29 &     3.20$\pm$   0.29 \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      0 &       99$\pm$      0 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      0 &      100$\pm$      0 \\ 
\foiii\        4960.29 & 
    71.6$\pm$    0.4 &     71.1$\pm$    0.4 & 
    56.0$\pm$    0.5 &     55.3$\pm$    0.5 & 
    97.5$\pm$    0.6 &     96.7$\pm$    0.6 & 
     104$\pm$      0 &      103$\pm$      0 \\ 
\foiii\       5008.24 & 
     215$\pm$      0 &      213$\pm$      0 & 
     172$\pm$      0 &      169$\pm$      0 & 
     290$\pm$      1 &      287$\pm$      1 & 
     311$\pm$      1 &      307$\pm$      1 \\ 
\fnii\       5756.24 & 
--- & --- & 
    0.72$\pm$   0.19 &     0.65$\pm$   0.17 & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    9.89$\pm$   0.13 &     9.28$\pm$   0.12 & 
    10.7$\pm$    0.2 &      9.6$\pm$    0.2 & 
    9.65$\pm$   0.19 &     9.02$\pm$   0.18 & 
    9.62$\pm$   0.19 &     8.90$\pm$   0.18 \\ 
\foi\        6302.05 & 
    3.67$\pm$   0.14 &     3.37$\pm$   0.13 & 
    6.54$\pm$   0.22 &     5.64$\pm$   0.19 & 
    5.85$\pm$   0.19 &     5.34$\pm$   0.17 & 
    4.42$\pm$   0.18 &     3.98$\pm$   0.16 \\ 
\fsiii\       6313.80 & 
    1.85$\pm$   0.10 &     1.70$\pm$   0.09 & 
    2.02$\pm$   0.15 &     1.74$\pm$   0.13 & 
    1.44$\pm$   0.13 &     1.31$\pm$   0.12 & 
    1.24$\pm$   0.13 &     1.12$\pm$   0.12 \\ 
\foi\       6365.54 & 
    1.15$\pm$   0.09 &     1.06$\pm$   0.08 & 
    2.07$\pm$   0.14 &     1.78$\pm$   0.12 & 
    1.87$\pm$   0.12 &     1.70$\pm$   0.11 & 
    1.24$\pm$   0.12 &     1.11$\pm$   0.11 \\ 
\ha\       6564.61 & 
     308$\pm$      1 &      280$\pm$      0 & 
     331$\pm$      1 &      280$\pm$      1 & 
     310$\pm$      1 &      280$\pm$      1 & 
     315$\pm$      1 &      279$\pm$      1 \\ 
\fnii\        6585.20 & 
    11.4$\pm$    0.1 &     10.3$\pm$    0.1 & 
    21.1$\pm$    0.2 &     17.8$\pm$    0.2 & 
    11.0$\pm$    0.1 &      9.9$\pm$    0.1 & 
    8.68$\pm$   0.14 &     7.70$\pm$   0.13 \\ 
\hei\        6679.99 & 
    2.75$\pm$   0.08 &     2.49$\pm$   0.08 & 
    2.95$\pm$   0.13 &     2.47$\pm$   0.11 & 
    2.96$\pm$   0.12 &     2.65$\pm$   0.10 & 
    2.60$\pm$   0.12 &     2.29$\pm$   0.11 \\ 
\fsii\       6718.29 & 
    26.7$\pm$    0.1 &     24.1$\pm$    0.1 & 
    42.1$\pm$    0.3 &     35.2$\pm$    0.2 & 
    28.8$\pm$    0.2 &     25.8$\pm$    0.2 & 
    23.8$\pm$    0.2 &     21.0$\pm$    0.2 \\ 
\fsii\       6732.67 & 
    18.6$\pm$    0.1 &     16.7$\pm$    0.1 & 
    29.9$\pm$    0.2 &     25.0$\pm$    0.2 & 
    20.2$\pm$    0.2 &     18.0$\pm$    0.2 & 
    16.8$\pm$    0.2 &     14.7$\pm$    0.2 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    6.40$\pm$   0.09 &     5.68$\pm$   0.08 & 
    7.85$\pm$   0.16 &     6.37$\pm$   0.13 & 
    6.62$\pm$   0.13 &     5.82$\pm$   0.11 & 
    5.68$\pm$   0.13 &     4.90$\pm$   0.11 \\ 
\foii\       7321.47 & 
    3.01$\pm$   0.09 &     2.65$\pm$   0.08 & 
    4.23$\pm$   0.16 &     3.39$\pm$   0.13 & 
    2.74$\pm$   0.13 &     2.39$\pm$   0.11 & 
    2.20$\pm$   0.13 &     1.88$\pm$   0.11 \\ 
\foii\       7332.25 & 
    2.56$\pm$   0.09 &     2.25$\pm$   0.08 & 
    3.47$\pm$   0.16 &     2.78$\pm$   0.13 & 
    2.20$\pm$   0.13 &     1.92$\pm$   0.11 & 
    1.34$\pm$   0.13 &     1.15$\pm$   0.11 \\ 
\fsiii\      9071.10 & 
    13.4$\pm$    0.1 &     11.2$\pm$    0.1 & 
    17.7$\pm$    0.2 &     12.9$\pm$    0.1 & 
    14.1$\pm$    0.2 &     11.7$\pm$    0.1 & 
    13.2$\pm$    0.2 &     10.6$\pm$    0.1 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    917$\pm$      2} & 
\multicolumn{2}{c|}{    517$\pm$      2} & 
\multicolumn{2}{c|}{    506$\pm$      2} & 
\multicolumn{2}{c|}{    542$\pm$      2} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   1249$\pm$      4} & 
\multicolumn{2}{c|}{    883$\pm$      4} & 
\multicolumn{2}{c|}{    704$\pm$      3} & 
\multicolumn{2}{c|}{    792$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.09$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.10$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.11$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> All_fluxes_combined1_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~4} & \multicolumn{2}{c|}{\hii\ Reg~5 }& \multicolumn{2}{c|}{\hii\ Reg~6} & \multicolumn{2}{c|}{\hii\ Reg~7} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
    2.03$\pm$   0.48 &     2.08$\pm$   0.49 \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      0 &      100$\pm$      0 \\ 
\foiii\        4960.29 & 
    71.7$\pm$    0.6 &     71.3$\pm$    0.6 & 
    60.5$\pm$    0.4 &     60.1$\pm$    0.4 & 
    95.0$\pm$    1.1 &     93.8$\pm$    1.1 & 
    60.3$\pm$    0.6 &     59.7$\pm$    0.6 \\ 
\foiii\       5008.24 & 
     215$\pm$      1 &      214$\pm$      1 & 
     179$\pm$      0 &      178$\pm$      0 & 
     291$\pm$      2 &      286$\pm$      2 & 
     178$\pm$      1 &      176$\pm$      1 \\ 
\fnii\       5756.24 & 
    0.61$\pm$   0.18 &     0.58$\pm$   0.17 & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    9.93$\pm$   0.22 &     9.51$\pm$   0.21 & 
    9.52$\pm$   0.20 &     8.94$\pm$   0.19 & 
    11.3$\pm$    0.5 &     10.1$\pm$    0.4 & 
    9.35$\pm$   0.31 &     8.56$\pm$   0.29 \\ 
\foi\        6302.05 & 
    5.03$\pm$   0.26 &     4.75$\pm$   0.24 & 
    6.05$\pm$   0.22 &     5.57$\pm$   0.20 & 
    6.99$\pm$   0.49 &     6.03$\pm$   0.42 & 
    7.33$\pm$   0.36 &     6.53$\pm$   0.32 \\ 
\fsiii\       6313.80 & 
    1.63$\pm$   0.17 &     1.54$\pm$   0.16 & 
    0.88$\pm$   0.15 &     0.81$\pm$   0.14 & 
    2.03$\pm$   0.33 &     1.75$\pm$   0.28 & 
    1.76$\pm$   0.23 &     1.57$\pm$   0.20 \\ 
\foi\       6365.54 & 
    1.38$\pm$   0.16 &     1.30$\pm$   0.15 & 
    1.99$\pm$   0.14 &     1.82$\pm$   0.13 & 
    2.38$\pm$   0.31 &     2.04$\pm$   0.27 & 
    1.88$\pm$   0.22 &     1.67$\pm$   0.19 \\ 
\ha\       6564.61 & 
     299$\pm$      1 &      280$\pm$      1 & 
     307$\pm$      1 &      279$\pm$      1 & 
     331$\pm$      2 &      280$\pm$      2 & 
     319$\pm$      2 &      280$\pm$      1 \\ 
\fnii\        6585.20 & 
    10.6$\pm$    0.2 &      9.9$\pm$    0.2 & 
    12.5$\pm$    0.2 &     11.4$\pm$    0.2 & 
    16.4$\pm$    0.3 &     13.8$\pm$    0.3 & 
    12.8$\pm$    0.2 &     11.2$\pm$    0.2 \\ 
\hei\        6679.99 & 
    3.01$\pm$   0.14 &     2.81$\pm$   0.13 & 
    2.56$\pm$   0.13 &     2.32$\pm$   0.12 & 
    2.86$\pm$   0.28 &     2.39$\pm$   0.24 & 
    2.67$\pm$   0.20 &     2.32$\pm$   0.18 \\ 
\fsii\       6718.29 & 
    27.3$\pm$    0.2 &     25.5$\pm$    0.2 & 
    33.8$\pm$    0.2 &     30.5$\pm$    0.2 & 
    34.7$\pm$    0.5 &     29.0$\pm$    0.4 & 
    35.3$\pm$    0.3 &     30.7$\pm$    0.3 \\ 
\fsii\       6732.67 & 
    19.4$\pm$    0.2 &     18.0$\pm$    0.2 & 
    23.5$\pm$    0.2 &     21.2$\pm$    0.2 & 
    24.6$\pm$    0.4 &     20.5$\pm$    0.3 & 
    24.6$\pm$    0.3 &     21.3$\pm$    0.2 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    6.07$\pm$   0.15 &     5.59$\pm$   0.13 & 
    5.43$\pm$   0.14 &     4.82$\pm$   0.12 & 
    8.84$\pm$   0.32 &     7.16$\pm$   0.26 & 
    4.85$\pm$   0.21 &     4.11$\pm$   0.18 \\ 
\foii\       7321.47 & 
    3.47$\pm$   0.15 &     3.18$\pm$   0.14 & 
    3.30$\pm$   0.14 &     2.91$\pm$   0.13 & 
    2.75$\pm$   0.31 &     2.20$\pm$   0.25 & 
    3.25$\pm$   0.22 &     2.73$\pm$   0.18 \\ 
\foii\       7332.25 & 
    2.81$\pm$   0.15 &     2.58$\pm$   0.13 & 
    2.44$\pm$   0.14 &     2.15$\pm$   0.12 & 
    3.14$\pm$   0.32 &     2.51$\pm$   0.26 & 
    3.56$\pm$   0.23 &     2.99$\pm$   0.19 \\ 
\fsiii\      9071.10 & 
    12.7$\pm$    0.2 &     11.2$\pm$    0.2 & 
    11.0$\pm$    0.2 &      9.2$\pm$    0.1 & 
    16.1$\pm$    0.4 &     11.7$\pm$    0.3 & 
    11.7$\pm$    0.3 &      9.1$\pm$    0.2 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    431$\pm$      2} & 
\multicolumn{2}{c|}{    557$\pm$      2} & 
\multicolumn{2}{c|}{    247$\pm$      2} & 
\multicolumn{2}{c|}{    365$\pm$      2} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    533$\pm$      2} & 
\multicolumn{2}{c|}{    754$\pm$      3} & 
\multicolumn{2}{c|}{    424$\pm$      3} & 
\multicolumn{2}{c|}{    559$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.06$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.09$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> All_fluxes_combined2_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~8} & \multicolumn{2}{c|}{\hii\ Reg~9 }& \multicolumn{2}{c|}{\hii\ Reg~10} & \multicolumn{2}{c|}{\hii\ Reg~11} \\
\hline\hline
\feiii\        4659.35 & 
    2.85$\pm$   0.92 &     2.91$\pm$   0.94 & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &       99$\pm$      1 \\ 
\foiii\        4960.29 & 
    39.0$\pm$    0.9 &     38.6$\pm$    0.9 & 
    97.4$\pm$    1.3 &     96.6$\pm$    1.3 & 
    20.3$\pm$    0.6 &     20.1$\pm$    0.6 & 
    45.5$\pm$    1.0 &     44.9$\pm$    1.0 \\ 
\foiii\       5008.24 & 
     114$\pm$      1 &      112$\pm$      1 & 
     287$\pm$      2 &      283$\pm$      2 & 
    62.5$\pm$    0.9 &     61.8$\pm$    0.8 & 
     139$\pm$      1 &      137$\pm$      1 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    6.73$\pm$   0.56 &     6.15$\pm$   0.51 & 
    10.4$\pm$    0.5 &      9.7$\pm$    0.5 & 
    7.65$\pm$   0.46 &     7.09$\pm$   0.43 & 
    9.97$\pm$   0.61 &     8.99$\pm$   0.55 \\ 
\foi\        6302.05 & 
    9.12$\pm$   0.63 &     8.09$\pm$   0.56 & 
    3.10$\pm$   0.53 &     2.80$\pm$   0.48 & 
    19.0$\pm$    0.5 &     17.1$\pm$    0.5 & 
    7.25$\pm$   0.69 &     6.32$\pm$   0.60 \\ 
\fsiii\       6313.80 & 
$<$   0.93  & $<$   0.82  & 
$<$   0.82  & $<$   0.74  & 
$<$   0.70  & $<$   0.64  & 
    2.74$\pm$   0.45 &     2.39$\pm$   0.39 \\ 
\foi\       6365.54 & 
    2.16$\pm$   0.42 &     1.91$\pm$   0.37 & 
    1.38$\pm$   0.36 &     1.24$\pm$   0.32 & 
    4.95$\pm$   0.34 &     4.45$\pm$   0.31 & 
    1.74$\pm$   0.43 &     1.51$\pm$   0.37 \\ 
\ha\       6564.61 & 
     320$\pm$      3 &      280$\pm$      3 & 
     315$\pm$      3 &      280$\pm$      2 & 
     314$\pm$      2 &      279$\pm$      2 & 
     327$\pm$      3 &      280$\pm$      3 \\ 
\fnii\        6585.20 & 
    16.3$\pm$    0.5 &     14.2$\pm$    0.4 & 
    9.12$\pm$   0.37 &     8.10$\pm$   0.33 & 
    18.2$\pm$    0.4 &     16.2$\pm$    0.3 & 
    13.4$\pm$    0.5 &     11.5$\pm$    0.4 \\ 
\hei\        6679.99 & 
    2.53$\pm$   0.37 &     2.20$\pm$   0.32 & 
    4.50$\pm$   0.33 &     3.97$\pm$   0.29 & 
    3.16$\pm$   0.29 &     2.80$\pm$   0.26 & 
    2.00$\pm$   0.41 &     1.69$\pm$   0.35 \\ 
\fsii\       6718.29 & 
    41.1$\pm$    0.6 &     35.5$\pm$    0.6 & 
    18.9$\pm$    0.4 &     16.7$\pm$    0.4 & 
    69.6$\pm$    0.7 &     61.5$\pm$    0.6 & 
    35.9$\pm$    0.6 &     30.3$\pm$    0.5 \\ 
\fsii\       6732.67 & 
    28.1$\pm$    0.5 &     24.3$\pm$    0.5 & 
    12.6$\pm$    0.4 &     11.1$\pm$    0.3 & 
    48.5$\pm$    0.5 &     42.8$\pm$    0.5 & 
    25.4$\pm$    0.5 &     21.4$\pm$    0.5 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    3.49$\pm$   0.38 &     2.95$\pm$   0.32 & 
    7.22$\pm$   0.34 &     6.24$\pm$   0.30 & 
    3.46$\pm$   0.31 &     2.99$\pm$   0.27 & 
    3.77$\pm$   0.43 &     3.10$\pm$   0.35 \\ 
\foii\       7321.47 & 
    3.52$\pm$   0.43 &     2.94$\pm$   0.36 & 
    2.78$\pm$   0.36 &     2.38$\pm$   0.31 & 
    3.28$\pm$   0.34 &     2.82$\pm$   0.29 & 
    3.86$\pm$   0.45 &     3.14$\pm$   0.37 \\ 
\foii\       7332.25 & 
    2.28$\pm$   0.44 &     1.90$\pm$   0.36 & 
$<$   0.49  & $<$   0.42  & 
    2.14$\pm$   0.34 &     1.83$\pm$   0.29 & 
    3.53$\pm$   0.47 &     2.87$\pm$   0.38 \\ 
\fsiii\      9071.10 & 
    11.2$\pm$    0.5 &      8.7$\pm$    0.4 & 
    15.1$\pm$    0.4 &     12.1$\pm$    0.3 & 
    7.29$\pm$   0.36 &     5.88$\pm$   0.29 & 
    12.5$\pm$    0.5 &      9.4$\pm$    0.4 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    143$\pm$      1} & 
\multicolumn{2}{c|}{    191$\pm$      1} & 
\multicolumn{2}{c|}{    234$\pm$      1} & 
\multicolumn{2}{c|}{    144$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    221$\pm$      2} & 
\multicolumn{2}{c|}{    278$\pm$      2} & 
\multicolumn{2}{c|}{    339$\pm$      2} & 
\multicolumn{2}{c|}{    237$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.11$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.11$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.15$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> All_fluxes_combined3_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~12} & \multicolumn{2}{c|}{\hii\ Reg~13 }& \multicolumn{2}{c|}{\hii\ Reg~14} & \multicolumn{2}{c|}{\hii\ Reg~15} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &       99$\pm$      1 \\ 
\foiii\        4960.29 & 
    73.3$\pm$    2.0 &     72.3$\pm$    2.0 & 
    60.0$\pm$    1.7 &     59.5$\pm$    1.7 & 
    37.3$\pm$    1.0 &     36.8$\pm$    1.0 & 
    41.3$\pm$    1.1 &     40.9$\pm$    1.1 \\ 
\foiii\       5008.24 & 
     219$\pm$      4 &      214$\pm$      4 & 
     175$\pm$      3 &      173$\pm$      3 & 
     103$\pm$      1 &      102$\pm$      1 & 
     130$\pm$      1 &      128$\pm$      1 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    13.1$\pm$    1.1 &     11.6$\pm$    1.0 & 
    8.38$\pm$   0.98 &     7.86$\pm$   0.92 & 
    8.63$\pm$   0.62 &     7.73$\pm$   0.55 & 
    10.8$\pm$    0.6 &      9.8$\pm$    0.6 \\ 
\foi\        6302.05 & 
    12.8$\pm$    1.2 &     10.9$\pm$    1.0 & 
    7.41$\pm$   1.06 &     6.81$\pm$   0.97 & 
    12.9$\pm$    0.7 &     11.1$\pm$    0.6 & 
    8.29$\pm$   0.76 &     7.28$\pm$   0.67 \\ 
\fsiii\       6313.80 & 
$<$   1.31  & $<$   1.12  & 
$<$   1.65  & $<$   1.52  & 
$<$   0.96  & $<$   0.83  & 
    2.55$\pm$   0.52 &     2.24$\pm$   0.46 \\ 
\foi\       6365.54 & 
--- & --- & 
    3.38$\pm$   0.70 &     3.10$\pm$   0.64 & 
    1.40$\pm$   0.46 &     1.20$\pm$   0.39 & 
--- & --- \\ 
\ha\       6564.61 & 
     337$\pm$      5 &      280$\pm$      4 & 
     308$\pm$      5 &      279$\pm$      4 & 
     330$\pm$      3 &      280$\pm$      3 & 
     324$\pm$      3 &      280$\pm$      3 \\ 
\fnii\        6585.20 & 
    24.2$\pm$    0.9 &     20.0$\pm$    0.7 & 
    12.1$\pm$    0.7 &     10.9$\pm$    0.6 & 
    15.1$\pm$    0.5 &     12.8$\pm$    0.4 & 
    17.9$\pm$    0.6 &     15.4$\pm$    0.5 \\ 
\hei\        6679.99 & 
    2.29$\pm$   0.70 &     1.89$\pm$   0.58 & 
--- & --- & 
    2.43$\pm$   0.40 &     2.04$\pm$   0.34 & 
    4.46$\pm$   0.45 &     3.82$\pm$   0.39 \\ 
\fsii\       6718.29 & 
    47.1$\pm$    1.1 &     38.6$\pm$    0.9 & 
    36.2$\pm$    0.9 &     32.7$\pm$    0.9 & 
    38.9$\pm$    0.6 &     32.5$\pm$    0.5 & 
    43.8$\pm$    0.7 &     37.4$\pm$    0.6 \\ 
\fsii\       6732.67 & 
    30.8$\pm$    0.9 &     25.3$\pm$    0.8 & 
    26.9$\pm$    0.8 &     24.3$\pm$    0.8 & 
    28.6$\pm$    0.5 &     23.9$\pm$    0.5 & 
    29.5$\pm$    0.6 &     25.1$\pm$    0.5 \\ 
\fneiii\        6870.16 & 
    4.48$\pm$   0.95 &     3.62$\pm$   0.77 & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    10.7$\pm$    0.7 &      8.5$\pm$    0.6 & 
    5.49$\pm$   0.68 &     4.87$\pm$   0.61 & 
    4.13$\pm$   0.42 &     3.36$\pm$   0.34 & 
    4.18$\pm$   0.45 &     3.48$\pm$   0.37 \\ 
\foii\       7321.47 & 
    6.02$\pm$   0.80 &     4.71$\pm$   0.63 & 
$<$   0.98  & $<$   0.87  & 
    2.27$\pm$   0.44 &     1.82$\pm$   0.35 & 
    2.80$\pm$   0.49 &     2.30$\pm$   0.41 \\ 
\foii\       7332.25 & 
    3.49$\pm$   0.80 &     2.73$\pm$   0.62 & 
    4.09$\pm$   0.76 &     3.60$\pm$   0.67 & 
    3.99$\pm$   0.47 &     3.20$\pm$   0.37 & 
    3.61$\pm$   0.49 &     2.97$\pm$   0.41 \\ 
\fsiii\      9071.10 & 
    16.9$\pm$    0.9 &     12.0$\pm$    0.6 & 
    14.8$\pm$    0.8 &     12.4$\pm$    0.7 & 
    10.4$\pm$    0.5 &      7.6$\pm$    0.4 & 
    11.1$\pm$    0.5 &      8.4$\pm$    0.4 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   73.7$\pm$    1.2} & 
\multicolumn{2}{c|}{   94.2$\pm$    1.5} & 
\multicolumn{2}{c|}{    172$\pm$      1} & 
\multicolumn{2}{c|}{    140$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    133$\pm$      2} & 
\multicolumn{2}{c|}{    127$\pm$      2} & 
\multicolumn{2}{c|}{    293$\pm$      3} & 
\multicolumn{2}{c|}{    224$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.18$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.09$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.14$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> All_fluxes_combined4_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~16} & \multicolumn{2}{c|}{\hii\ Reg~17 }& \multicolumn{2}{c|}{\hii\ Reg~18} & \multicolumn{2}{c|}{\hii\ Reg~19} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      1 &       99$\pm$      1 \\ 
\foiii\        4960.29 & 
    38.7$\pm$    0.8 &     38.5$\pm$    0.8 & 
    48.3$\pm$    1.5 &     47.8$\pm$    1.5 & 
    56.0$\pm$    2.2 &     55.1$\pm$    2.2 & 
    9.97$\pm$   0.87 &     9.87$\pm$   0.86 \\ 
\foiii\       5008.24 & 
     112$\pm$      1 &      111$\pm$      1 & 
     132$\pm$      2 &      130$\pm$      2 & 
     155$\pm$      3 &      151$\pm$      3 & 
    37.0$\pm$    1.0 &     36.4$\pm$    1.0 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    8.69$\pm$   0.54 &     8.24$\pm$   0.52 & 
    8.87$\pm$   0.92 &     8.10$\pm$   0.84 & 
    13.8$\pm$    1.3 &     12.0$\pm$    1.2 & 
    6.99$\pm$   0.66 &     6.38$\pm$   0.60 \\ 
\foi\        6302.05 & 
    8.00$\pm$   0.66 &     7.45$\pm$   0.62 & 
    10.1$\pm$    1.1 &      9.0$\pm$    0.9 & 
    16.2$\pm$    1.6 &     13.5$\pm$    1.4 & 
    9.84$\pm$   0.75 &     8.72$\pm$   0.66 \\ 
\fsiii\       6313.80 & 
$<$   0.64  & $<$   0.60  & 
$<$   1.02  & $<$   0.90  & 
$<$   1.61  & $<$   1.34  & 
$<$   1.12  & $<$   0.99  \\ 
\foi\       6365.54 & 
    2.84$\pm$   0.42 &     2.64$\pm$   0.39 & 
    3.56$\pm$   0.65 &     3.14$\pm$   0.58 & 
    5.94$\pm$   1.07 &     4.92$\pm$   0.88 & 
    2.29$\pm$   0.51 &     2.02$\pm$   0.45 \\ 
\ha\       6564.61 & 
     303$\pm$      2 &      280$\pm$      2 & 
     320$\pm$      5 &      280$\pm$      4 & 
     344$\pm$      7 &      279$\pm$      5 & 
     321$\pm$      3 &      280$\pm$      3 \\ 
\fnii\        6585.20 & 
    13.9$\pm$    0.4 &     12.8$\pm$    0.4 & 
    9.35$\pm$   0.62 &     8.15$\pm$   0.54 & 
    21.6$\pm$    1.1 &     17.5$\pm$    0.9 & 
    17.2$\pm$    0.5 &     14.9$\pm$    0.5 \\ 
\hei\        6679.99 & 
    2.61$\pm$   0.36 &     2.40$\pm$   0.33 & 
    3.23$\pm$   0.57 &     2.80$\pm$   0.49 & 
    3.21$\pm$   0.95 &     2.58$\pm$   0.77 & 
    2.69$\pm$   0.45 &     2.33$\pm$   0.39 \\ 
\fsii\       6718.29 & 
    38.5$\pm$    0.6 &     35.3$\pm$    0.5 & 
    36.2$\pm$    0.9 &     31.3$\pm$    0.7 & 
    59.8$\pm$    1.6 &     47.9$\pm$    1.3 & 
    53.6$\pm$    0.8 &     46.3$\pm$    0.7 \\ 
\fsii\       6732.67 & 
    26.4$\pm$    0.5 &     24.2$\pm$    0.4 & 
    25.5$\pm$    0.7 &     22.0$\pm$    0.6 & 
    40.2$\pm$    1.3 &     32.1$\pm$    1.1 & 
    38.1$\pm$    0.7 &     32.9$\pm$    0.6 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
    5.32$\pm$   1.28 &     4.20$\pm$   1.01 & 
    1.76$\pm$   0.57 &     1.50$\pm$   0.49 \\ 
\fariii\       7137.80 & 
    4.44$\pm$   0.37 &     4.01$\pm$   0.34 & 
    4.70$\pm$   0.63 &     3.97$\pm$   0.53 & 
    3.39$\pm$   0.97 &     2.62$\pm$   0.75 & 
    1.83$\pm$   0.45 &     1.54$\pm$   0.38 \\ 
\foii\       7321.47 & 
    2.34$\pm$   0.40 &     2.10$\pm$   0.36 & 
    2.40$\pm$   0.67 &     2.00$\pm$   0.56 & 
$<$   2.05  & $<$   1.56  & 
    2.95$\pm$   0.52 &     2.46$\pm$   0.43 \\ 
\foii\       7332.25 & 
$<$   0.86  & $<$   0.78  & 
    4.25$\pm$   0.70 &     3.55$\pm$   0.58 & 
$<$   3.59  & $<$   2.73  & 
$<$   0.93  & $<$   0.78  \\ 
\fsiii\      9071.10 & 
    9.26$\pm$   0.44 &     7.98$\pm$   0.38 & 
    7.23$\pm$   0.67 &     5.62$\pm$   0.52 & 
    12.8$\pm$    1.1 &      8.7$\pm$    0.8 & 
    5.80$\pm$   0.53 &     4.49$\pm$   0.41 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    168$\pm$      1} & 
\multicolumn{2}{c|}{    107$\pm$      1} & 
\multicolumn{2}{c|}{   70.9$\pm$    1.4} & 
\multicolumn{2}{c|}{    151$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    217$\pm$      2} & 
\multicolumn{2}{c|}{    166$\pm$      2} & 
\multicolumn{2}{c|}{    137$\pm$      3} & 
\multicolumn{2}{c|}{    235$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.08$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.20$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> All_fluxes_combined5_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~20} & \multicolumn{2}{c|}{\hii\ Reg~21 }& \multicolumn{2}{c|}{\hii\ Reg~22} & \multicolumn{2}{c|}{\hii\ Reg~23} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
    7.49$\pm$   2.02 &     7.55$\pm$   2.04 & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 \\ 
\foiii\        4960.29 & 
    25.6$\pm$    1.0 &     25.4$\pm$    1.0 & 
    39.8$\pm$    1.8 &     39.1$\pm$    1.8 & 
    50.0$\pm$    2.2 &     49.7$\pm$    2.2 & 
    35.3$\pm$    1.5 &     34.9$\pm$    1.5 \\ 
\foiii\       5008.24 & 
    77.2$\pm$    1.4 &     76.2$\pm$    1.3 & 
     111$\pm$      2 &      108$\pm$      2 & 
     133$\pm$      3 &      132$\pm$      3 & 
     113$\pm$      2 &      112$\pm$      2 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    11.1$\pm$    0.7 &     10.3$\pm$    0.7 & 
    6.53$\pm$   1.18 &     5.60$\pm$   1.01 & 
    9.00$\pm$   1.31 &     8.49$\pm$   1.24 & 
    9.72$\pm$   0.97 &     8.93$\pm$   0.89 \\ 
\foi\        6302.05 & 
    10.5$\pm$    0.8 &      9.4$\pm$    0.7 & 
    29.1$\pm$    1.5 &     23.7$\pm$    1.2 & 
    11.2$\pm$    1.5 &     10.3$\pm$    1.4 & 
    9.89$\pm$   1.17 &     8.83$\pm$   1.04 \\ 
\fsiii\       6313.80 & 
$<$   0.79  & $<$   0.71  & 
$<$   1.28  & $<$   1.04  & 
$<$   2.21  & $<$   2.05  & 
$<$   1.70  & $<$   1.52  \\ 
\foi\       6365.54 & 
--- & --- & 
    9.87$\pm$   0.93 &     7.97$\pm$   0.75 & 
    3.17$\pm$   1.01 &     2.93$\pm$   0.93 & 
--- & --- \\ 
\ha\       6564.61 & 
     315$\pm$      3 &      280$\pm$      3 & 
     354$\pm$      6 &      280$\pm$      5 & 
     305$\pm$      6 &      280$\pm$      6 & 
     318$\pm$      5 &      280$\pm$      4 \\ 
\fnii\        6585.20 & 
    15.4$\pm$    0.6 &     13.6$\pm$    0.5 & 
    25.8$\pm$    1.0 &     20.3$\pm$    0.8 & 
    12.0$\pm$    1.0 &     11.0$\pm$    0.9 & 
    16.9$\pm$    0.8 &     14.8$\pm$    0.7 \\ 
\hei\        6679.99 & 
    1.88$\pm$   0.49 &     1.66$\pm$   0.43 & 
    3.67$\pm$   0.79 &     2.87$\pm$   0.62 & 
--- & --- & 
    3.31$\pm$   0.70 &     2.89$\pm$   0.61 \\ 
\fsii\       6718.29 & 
    48.1$\pm$    0.8 &     42.2$\pm$    0.7 & 
    87.6$\pm$    1.9 &     68.2$\pm$    1.5 & 
    31.7$\pm$    1.2 &     28.8$\pm$    1.1 & 
    40.3$\pm$    1.0 &     35.1$\pm$    0.9 \\ 
\fsii\       6732.67 & 
    33.4$\pm$    0.7 &     29.4$\pm$    0.6 & 
    61.8$\pm$    1.5 &     48.0$\pm$    1.2 & 
    24.8$\pm$    1.1 &     22.6$\pm$    1.0 & 
    29.0$\pm$    0.9 &     25.2$\pm$    0.8 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
    2.73$\pm$   0.89 &     2.36$\pm$   0.77 \\ 
\fariii\       7137.80 & 
    4.01$\pm$   0.50 &     3.45$\pm$   0.43 & 
    3.69$\pm$   0.82 &     2.75$\pm$   0.61 & 
    6.38$\pm$   0.89 &     5.72$\pm$   0.80 & 
    5.25$\pm$   0.67 &     4.47$\pm$   0.57 \\ 
\foii\       7321.47 & 
    3.70$\pm$   0.53 &     3.16$\pm$   0.45 & 
    4.68$\pm$   0.90 &     3.43$\pm$   0.66 & 
$<$   1.97  & $<$   1.75  & 
    3.79$\pm$   0.72 &     3.20$\pm$   0.61 \\ 
\foii\       7332.25 & 
    4.29$\pm$   0.54 &     3.65$\pm$   0.46 & 
$<$   1.88  & $<$   1.38  & 
$<$   1.56  & $<$   1.38  & 
$<$   1.53  & $<$   1.29  \\ 
\fsiii\      9071.10 & 
    8.33$\pm$   0.55 &     6.66$\pm$   0.44 & 
    11.3$\pm$    0.9 &      7.3$\pm$    0.6 & 
    12.7$\pm$    1.0 &     10.8$\pm$    0.9 & 
    12.7$\pm$    0.8 &     10.0$\pm$    0.6 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    147$\pm$      1} & 
\multicolumn{2}{c|}{   90.4$\pm$    1.7} & 
\multicolumn{2}{c|}{   66.3$\pm$    1.4} & 
\multicolumn{2}{c|}{   91.9$\pm$    1.4} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    216$\pm$      2} & 
\multicolumn{2}{c|}{    191$\pm$      4} & 
\multicolumn{2}{c|}{   87.9$\pm$    1.9} & 
\multicolumn{2}{c|}{    138$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.12$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.23$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.08$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.12$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> All_fluxes_combined6_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~24} & \multicolumn{2}{c|}{\hii\ Reg~25 }& \multicolumn{2}{c|}{\hii\ Reg~26} & \multicolumn{2}{c|}{\hii\ Reg~27} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
    7.23$\pm$   2.29 &     7.48$\pm$   2.37 & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      3 &      100$\pm$      3 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      2 &      100$\pm$      2 \\ 
\foiii\        4960.29 & 
    73.2$\pm$    2.0 &     71.9$\pm$    2.0 & 
    32.3$\pm$    2.0 &     31.8$\pm$    2.0 & 
     110$\pm$      2 &      109$\pm$      2 & 
    34.2$\pm$    1.4 &     33.7$\pm$    1.4 \\ 
\foiii\       5008.24 & 
     227$\pm$      4 &      221$\pm$      4 & 
    73.5$\pm$    2.5 &     71.9$\pm$    2.5 & 
     335$\pm$      5 &      330$\pm$      4 & 
     108$\pm$      2 &      106$\pm$      2 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    10.4$\pm$    1.1 &      8.9$\pm$    0.9 & 
    5.17$\pm$   1.30 &     4.52$\pm$   1.14 & 
    11.1$\pm$    0.9 &     10.0$\pm$    0.8 & 
    9.45$\pm$   1.00 &     8.32$\pm$   0.88 \\ 
\foi\        6302.05 & 
    8.22$\pm$   1.22 &     6.68$\pm$   0.99 & 
    20.3$\pm$    1.7 &     16.9$\pm$    1.4 & 
    12.8$\pm$    1.1 &     11.1$\pm$    0.9 & 
    16.1$\pm$    1.1 &     13.6$\pm$    0.9 \\ 
\fsiii\       6313.80 & 
$<$   1.22  & $<$   0.99  & 
$<$   2.28  & $<$   1.91  & 
    3.84$\pm$   0.70 &     3.32$\pm$   0.61 & 
$<$   1.10  & $<$   0.92  \\ 
\foi\       6365.54 & 
--- & --- & 
    4.72$\pm$   1.00 &     3.92$\pm$   0.83 & 
    3.22$\pm$   0.69 &     2.78$\pm$   0.59 & 
    5.54$\pm$   0.71 &     4.65$\pm$   0.60 \\ 
\ha\       6564.61 & 
     354$\pm$      6 &      280$\pm$      5 & 
     343$\pm$      7 &      280$\pm$      6 & 
     329$\pm$      4 &      280$\pm$      4 & 
     339$\pm$      5 &      279$\pm$      4 \\ 
\fnii\        6585.20 & 
    17.7$\pm$    0.8 &     14.0$\pm$    0.7 & 
    14.3$\pm$    1.0 &     11.7$\pm$    0.8 & 
    16.1$\pm$    0.7 &     13.7$\pm$    0.6 & 
    24.4$\pm$    0.8 &     20.1$\pm$    0.7 \\ 
\hei\        6679.99 & 
    3.49$\pm$   0.71 &     2.72$\pm$   0.56 & 
--- & --- & 
    1.92$\pm$   0.60 &     1.62$\pm$   0.51 & 
    4.33$\pm$   0.65 &     3.53$\pm$   0.53 \\ 
\fsii\       6718.29 & 
    40.3$\pm$    1.1 &     31.3$\pm$    0.8 & 
    59.9$\pm$    1.6 &     48.2$\pm$    1.3 & 
    42.8$\pm$    0.9 &     36.0$\pm$    0.8 & 
    64.7$\pm$    1.3 &     52.6$\pm$    1.1 \\ 
\fsii\       6732.67 & 
    27.8$\pm$    0.9 &     21.6$\pm$    0.7 & 
    41.0$\pm$    1.3 &     32.9$\pm$    1.1 & 
    33.6$\pm$    0.8 &     28.2$\pm$    0.7 & 
    45.0$\pm$    1.0 &     36.5$\pm$    0.8 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
    3.74$\pm$   0.91 &     3.00$\pm$   0.73 \\ 
\fariii\       7137.80 & 
    6.80$\pm$   0.72 &     5.07$\pm$   0.54 & 
--- & --- & 
    7.91$\pm$   0.62 &     6.46$\pm$   0.50 & 
    7.23$\pm$   0.70 &     5.69$\pm$   0.55 \\ 
\foii\       7321.47 & 
    3.31$\pm$   0.75 &     2.43$\pm$   0.55 & 
    5.77$\pm$   1.02 &     4.40$\pm$   0.78 & 
    3.95$\pm$   0.63 &     3.19$\pm$   0.51 & 
$<$   1.51  & $<$   1.17  \\ 
\foii\       7332.25 & 
$<$   1.13  & $<$   0.83  & 
    4.66$\pm$   1.00 &     3.55$\pm$   0.76 & 
    3.87$\pm$   0.64 &     3.12$\pm$   0.52 & 
$<$   2.70  & $<$   2.09  \\ 
\fsiii\      9071.10 & 
    16.3$\pm$    0.9 &     10.5$\pm$    0.6 & 
    7.15$\pm$   1.03 &     4.89$\pm$   0.71 & 
    15.3$\pm$    0.7 &     11.3$\pm$    0.5 & 
    13.9$\pm$    0.8 &      9.7$\pm$    0.5 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   89.8$\pm$    1.6} & 
\multicolumn{2}{c|}{   71.5$\pm$    1.5} & 
\multicolumn{2}{c|}{    109$\pm$      1} & 
\multicolumn{2}{c|}{    106$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    190$\pm$      4} & 
\multicolumn{2}{c|}{    137$\pm$      3} & 
\multicolumn{2}{c|}{    183$\pm$      2} & 
\multicolumn{2}{c|}{    196$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.23$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.20$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.19$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> All_fluxes_combined7_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. } \\
 & \multicolumn{2}{c|}{\hii\ Reg~28} & \multicolumn{2}{c|}{\hii\ Reg~29 } \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      3 &      100$\pm$      3 & 
     100$\pm$      2 &      100$\pm$      2 \\ 
\foiii\        4960.29 & 
    31.2$\pm$    2.4 &     30.8$\pm$    2.3 & 
    20.5$\pm$    1.3 &     20.2$\pm$    1.2 \\ 
\foiii\       5008.24 & 
     103$\pm$      3 &      101$\pm$      3 & 
    58.4$\pm$    1.5 &     57.2$\pm$    1.5 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    10.1$\pm$    1.6 &      9.0$\pm$    1.4 & 
    7.60$\pm$   0.91 &     6.66$\pm$   0.80 \\ 
\foi\        6302.05 & 
    13.1$\pm$    2.0 &     11.4$\pm$    1.7 & 
    12.4$\pm$    1.0 &     10.4$\pm$    0.9 \\ 
\fsiii\       6313.80 & 
$<$   1.97  & $<$   1.70  & 
$<$   1.59  & $<$   1.33  \\ 
\foi\       6365.54 & 
--- & --- & 
--- & --- \\ 
\ha\       6564.61 & 
     330$\pm$      8 &      280$\pm$      7 & 
     342$\pm$      5 &      279$\pm$      4 \\ 
\fnii\        6585.20 & 
    12.7$\pm$    1.3 &     10.8$\pm$    1.1 & 
    20.5$\pm$    0.7 &     16.8$\pm$    0.6 \\ 
\hei\        6679.99 & 
--- & --- & 
    3.10$\pm$   0.61 &     2.51$\pm$   0.50 \\ 
\fsii\       6718.29 & 
    26.5$\pm$    1.4 &     22.2$\pm$    1.2 & 
    57.3$\pm$    1.1 &     46.3$\pm$    0.9 \\ 
\fsii\       6732.67 & 
    16.9$\pm$    1.2 &     14.1$\pm$    1.0 & 
    39.3$\pm$    0.9 &     31.7$\pm$    0.7 \\ 
\fneiii\        6870.16 & 
    5.16$\pm$   1.46 &     4.28$\pm$   1.21 & 
--- & --- \\ 
\fariii\       7137.80 & 
    3.89$\pm$   1.06 &     3.17$\pm$   0.87 & 
    2.67$\pm$   0.63 &     2.08$\pm$   0.49 \\ 
\foii\       7321.47 & 
$<$   2.36  & $<$   1.90  & 
$<$   0.98  & $<$   0.75  \\ 
\foii\       7332.25 & 
    8.10$\pm$   1.18 &     6.50$\pm$   0.95 & 
$<$   1.10  & $<$   0.84  \\ 
\fsiii\      9071.10 & 
    13.8$\pm$    1.4 &     10.2$\pm$    1.0 & 
    11.0$\pm$    0.7 &      7.6$\pm$    0.5 \\ 
 & & & &  \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   48.9$\pm$    1.2} & 
\multicolumn{2}{c|}{    109$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   82.8$\pm$    2.3} & 
\multicolumn{2}{c|}{    207$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.19$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/ALL_SFR_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|c|cc|}
\hline
\hii\ Region ID & $L$(\ha) ($\times10^{36}$ erg\,s$^{-1}$) & SFR(\ha) ($\times10^{-2}$ \Msol \,yr$^{-1}$) \\
\hline
0 & 129.46 $\pm$   0.16 &   0.47 $\pm$   0.11 \\%  18.00  0.000207
1 &  91.51 $\pm$   0.18 &   0.38 $\pm$   0.09 \\%  18.00  0.000217
2 &  72.99 $\pm$   0.12 &   0.33 $\pm$   0.08 \\%  18.00  0.000189
3 &  82.11 $\pm$   0.14 &   0.36 $\pm$   0.08 \\%  18.00  0.000174
4 &  55.30 $\pm$   0.10 &   0.28 $\pm$   0.07 \\%  18.00  0.000189
5 &  78.23 $\pm$   0.13 &   0.35 $\pm$   0.08 \\%  18.00  0.000185
6 &  43.97 $\pm$   0.15 &   0.24 $\pm$   0.06 \\%  18.00  0.000243
7 &  57.96 $\pm$   0.13 &   0.29 $\pm$   0.07 \\%  18.00  0.000276
8 &  23.00 $\pm$   0.09 &   0.16 $\pm$   0.04 \\%  18.00  0.000158
9 &  28.83 $\pm$   0.09 &   0.19 $\pm$   0.05 \\%  18.00  0.000176
10 &  35.13 $\pm$   0.10 &   0.21 $\pm$   0.05 \\%  18.00  0.000197
11 &  24.66 $\pm$   0.10 &   0.17 $\pm$   0.04 \\%  18.00  0.000262
12 &  13.81 $\pm$   0.10 &   0.12 $\pm$   0.04 \\%  18.00  0.000216
13 &  13.26 $\pm$   0.06 &   0.12 $\pm$   0.04 \\%  18.00  0.000168
14 &  30.42 $\pm$   0.13 &   0.19 $\pm$   0.05 \\%  18.00  0.000282
15 &  23.29 $\pm$   0.10 &   0.16 $\pm$   0.04 \\%  18.00  0.000197
16 &  22.54 $\pm$   0.07 &   0.16 $\pm$   0.04 \\%  18.00  0.000214
17 &  17.24 $\pm$   0.09 &   0.14 $\pm$   0.04 \\%  18.00  0.000243
18 &  14.25 $\pm$   0.13 &   0.12 $\pm$   0.04 \\%  18.00  0.000205
19 &  24.39 $\pm$   0.10 &   0.17 $\pm$   0.04 \\%  18.00  0.000150
20 &  22.48 $\pm$   0.09 &   0.16 $\pm$   0.04 \\%  18.00  0.000220
21 &  19.82 $\pm$   0.18 &   0.15 $\pm$   0.04 \\%  18.00  0.000220
22 &   9.10 $\pm$   0.05 &   0.09 $\pm$   0.03 \\%  18.00  0.000180
23 &  14.38 $\pm$   0.08 &   0.12 $\pm$   0.04 \\%  18.00  0.000199
24 &  19.71 $\pm$   0.18 &   0.15 $\pm$   0.04 \\%  18.00  0.000248
25 &  14.25 $\pm$   0.14 &   0.12 $\pm$   0.04 \\%  18.00  0.000197
26 &  19.03 $\pm$   0.11 &   0.14 $\pm$   0.04 \\%  18.00  0.000237
27 &  20.40 $\pm$   0.14 &   0.15 $\pm$   0.04 \\%  18.00  0.000212
28 &   8.58 $\pm$   0.08 &   0.09 $\pm$   0.03 \\%  18.00  0.000201
29 &  21.48 $\pm$   0.14 &   0.16 $\pm$   0.04 \\%  18.00  0.000164
\hline
\end{tabular}
\label{tab:SFR}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined0_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~0} & \multicolumn{2}{c|}{\hii\ Reg~1 }& \multicolumn{2}{c|}{\hii\ Reg~2} & \multicolumn{2}{c|}{\hii\ Reg~3} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
    3.71$\pm$   0.29 &     3.77$\pm$   0.29 & 
    3.15$\pm$   0.29 &     3.20$\pm$   0.29 \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      0 &       99$\pm$      0 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      0 &      100$\pm$      0 \\ 
\foiii\        4960.29 & 
    71.6$\pm$    0.4 &     71.1$\pm$    0.4 & 
    56.0$\pm$    0.5 &     55.3$\pm$    0.5 & 
    97.5$\pm$    0.6 &     96.7$\pm$    0.6 & 
     104$\pm$      0 &      103$\pm$      0 \\ 
\foiii\       5008.24 & 
     215$\pm$      0 &      213$\pm$      0 & 
     172$\pm$      0 &      169$\pm$      0 & 
     290$\pm$      1 &      287$\pm$      1 & 
     311$\pm$      1 &      307$\pm$      1 \\ 
\fnii\       5756.24 & 
--- & --- & 
    0.72$\pm$   0.19 &     0.65$\pm$   0.17 & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    9.89$\pm$   0.13 &     9.28$\pm$   0.12 & 
    10.7$\pm$    0.2 &      9.6$\pm$    0.2 & 
    9.65$\pm$   0.19 &     9.02$\pm$   0.18 & 
    9.62$\pm$   0.19 &     8.90$\pm$   0.18 \\ 
\foi\        6302.05 & 
    3.67$\pm$   0.14 &     3.37$\pm$   0.13 & 
    6.54$\pm$   0.22 &     5.64$\pm$   0.19 & 
    5.85$\pm$   0.19 &     5.34$\pm$   0.17 & 
    4.42$\pm$   0.18 &     3.98$\pm$   0.16 \\ 
\fsiii\       6313.80 & 
    1.85$\pm$   0.10 &     1.70$\pm$   0.09 & 
    2.02$\pm$   0.15 &     1.74$\pm$   0.13 & 
    1.44$\pm$   0.13 &     1.31$\pm$   0.12 & 
    1.24$\pm$   0.13 &     1.12$\pm$   0.12 \\ 
\foi\       6365.54 & 
    1.15$\pm$   0.09 &     1.06$\pm$   0.08 & 
    2.07$\pm$   0.14 &     1.78$\pm$   0.12 & 
    1.87$\pm$   0.12 &     1.70$\pm$   0.11 & 
    1.24$\pm$   0.12 &     1.11$\pm$   0.11 \\ 
\ha\       6564.61 & 
     308$\pm$      1 &      280$\pm$      0 & 
     331$\pm$      1 &      280$\pm$      1 & 
     310$\pm$      1 &      280$\pm$      1 & 
     315$\pm$      1 &      279$\pm$      1 \\ 
\fnii\        6585.20 & 
    11.4$\pm$    0.1 &     10.3$\pm$    0.1 & 
    21.1$\pm$    0.2 &     17.8$\pm$    0.2 & 
    11.0$\pm$    0.1 &      9.9$\pm$    0.1 & 
    8.68$\pm$   0.14 &     7.70$\pm$   0.13 \\ 
\hei\        6679.99 & 
    2.75$\pm$   0.08 &     2.49$\pm$   0.08 & 
    2.95$\pm$   0.13 &     2.47$\pm$   0.11 & 
    2.96$\pm$   0.12 &     2.65$\pm$   0.10 & 
    2.60$\pm$   0.12 &     2.29$\pm$   0.11 \\ 
\fsii\       6718.29 & 
    26.7$\pm$    0.1 &     24.1$\pm$    0.1 & 
    42.1$\pm$    0.3 &     35.2$\pm$    0.2 & 
    28.8$\pm$    0.2 &     25.8$\pm$    0.2 & 
    23.8$\pm$    0.2 &     21.0$\pm$    0.2 \\ 
\fsii\       6732.67 & 
    18.6$\pm$    0.1 &     16.7$\pm$    0.1 & 
    29.9$\pm$    0.2 &     25.0$\pm$    0.2 & 
    20.2$\pm$    0.2 &     18.0$\pm$    0.2 & 
    16.8$\pm$    0.2 &     14.7$\pm$    0.2 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    6.40$\pm$   0.09 &     5.68$\pm$   0.08 & 
    7.85$\pm$   0.16 &     6.37$\pm$   0.13 & 
    6.62$\pm$   0.13 &     5.82$\pm$   0.11 & 
    5.68$\pm$   0.13 &     4.90$\pm$   0.11 \\ 
\foii\       7321.47 & 
    3.01$\pm$   0.09 &     2.65$\pm$   0.08 & 
    4.23$\pm$   0.16 &     3.39$\pm$   0.13 & 
    2.74$\pm$   0.13 &     2.39$\pm$   0.11 & 
    2.20$\pm$   0.13 &     1.88$\pm$   0.11 \\ 
\foii\       7332.25 & 
    2.56$\pm$   0.09 &     2.25$\pm$   0.08 & 
    3.47$\pm$   0.16 &     2.78$\pm$   0.13 & 
    2.20$\pm$   0.13 &     1.92$\pm$   0.11 & 
    1.34$\pm$   0.13 &     1.15$\pm$   0.11 \\ 
\fsiii\      9071.10 & 
    13.4$\pm$    0.1 &     11.2$\pm$    0.1 & 
    17.7$\pm$    0.2 &     12.9$\pm$    0.1 & 
    14.1$\pm$    0.2 &     11.7$\pm$    0.1 & 
    13.2$\pm$    0.2 &     10.6$\pm$    0.1 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    917$\pm$      2} & 
\multicolumn{2}{c|}{    517$\pm$      2} & 
\multicolumn{2}{c|}{    506$\pm$      2} & 
\multicolumn{2}{c|}{    542$\pm$      2} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   1249$\pm$      4} & 
\multicolumn{2}{c|}{    883$\pm$      4} & 
\multicolumn{2}{c|}{    704$\pm$      3} & 
\multicolumn{2}{c|}{    792$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.09$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.10$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.11$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined1_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~4} & \multicolumn{2}{c|}{\hii\ Reg~5 }& \multicolumn{2}{c|}{\hii\ Reg~6} & \multicolumn{2}{c|}{\hii\ Reg~7} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
    2.03$\pm$   0.48 &     2.08$\pm$   0.49 \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      0 &      100$\pm$      0 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      0 &      100$\pm$      0 \\ 
\foiii\        4960.29 & 
    71.7$\pm$    0.6 &     71.3$\pm$    0.6 & 
    60.5$\pm$    0.4 &     60.1$\pm$    0.4 & 
    95.0$\pm$    1.1 &     93.8$\pm$    1.1 & 
    60.3$\pm$    0.6 &     59.7$\pm$    0.6 \\ 
\foiii\       5008.24 & 
     215$\pm$      1 &      214$\pm$      1 & 
     179$\pm$      0 &      178$\pm$      0 & 
     291$\pm$      2 &      286$\pm$      2 & 
     178$\pm$      1 &      176$\pm$      1 \\ 
\fnii\       5756.24 & 
    0.61$\pm$   0.18 &     0.58$\pm$   0.17 & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    9.93$\pm$   0.22 &     9.51$\pm$   0.21 & 
    9.52$\pm$   0.20 &     8.94$\pm$   0.19 & 
    11.3$\pm$    0.5 &     10.1$\pm$    0.4 & 
    9.35$\pm$   0.31 &     8.56$\pm$   0.29 \\ 
\foi\        6302.05 & 
    5.03$\pm$   0.26 &     4.75$\pm$   0.24 & 
    6.05$\pm$   0.22 &     5.57$\pm$   0.20 & 
    6.99$\pm$   0.49 &     6.03$\pm$   0.42 & 
    7.33$\pm$   0.36 &     6.53$\pm$   0.32 \\ 
\fsiii\       6313.80 & 
    1.63$\pm$   0.17 &     1.54$\pm$   0.16 & 
    0.88$\pm$   0.15 &     0.81$\pm$   0.14 & 
    2.03$\pm$   0.33 &     1.75$\pm$   0.28 & 
    1.76$\pm$   0.23 &     1.57$\pm$   0.20 \\ 
\foi\       6365.54 & 
    1.38$\pm$   0.16 &     1.30$\pm$   0.15 & 
    1.99$\pm$   0.14 &     1.82$\pm$   0.13 & 
    2.38$\pm$   0.31 &     2.04$\pm$   0.27 & 
    1.88$\pm$   0.22 &     1.67$\pm$   0.19 \\ 
\ha\       6564.61 & 
     299$\pm$      1 &      280$\pm$      1 & 
     307$\pm$      1 &      279$\pm$      1 & 
     331$\pm$      2 &      280$\pm$      2 & 
     319$\pm$      2 &      280$\pm$      1 \\ 
\fnii\        6585.20 & 
    10.6$\pm$    0.2 &      9.9$\pm$    0.2 & 
    12.5$\pm$    0.2 &     11.4$\pm$    0.2 & 
    16.4$\pm$    0.3 &     13.8$\pm$    0.3 & 
    12.8$\pm$    0.2 &     11.2$\pm$    0.2 \\ 
\hei\        6679.99 & 
    3.01$\pm$   0.14 &     2.81$\pm$   0.13 & 
    2.56$\pm$   0.13 &     2.32$\pm$   0.12 & 
    2.86$\pm$   0.28 &     2.39$\pm$   0.24 & 
    2.67$\pm$   0.20 &     2.32$\pm$   0.18 \\ 
\fsii\       6718.29 & 
    27.3$\pm$    0.2 &     25.5$\pm$    0.2 & 
    33.8$\pm$    0.2 &     30.5$\pm$    0.2 & 
    34.7$\pm$    0.5 &     29.0$\pm$    0.4 & 
    35.3$\pm$    0.3 &     30.7$\pm$    0.3 \\ 
\fsii\       6732.67 & 
    19.4$\pm$    0.2 &     18.0$\pm$    0.2 & 
    23.5$\pm$    0.2 &     21.2$\pm$    0.2 & 
    24.6$\pm$    0.4 &     20.5$\pm$    0.3 & 
    24.6$\pm$    0.3 &     21.3$\pm$    0.2 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    6.07$\pm$   0.15 &     5.59$\pm$   0.13 & 
    5.43$\pm$   0.14 &     4.82$\pm$   0.12 & 
    8.84$\pm$   0.32 &     7.16$\pm$   0.26 & 
    4.85$\pm$   0.21 &     4.11$\pm$   0.18 \\ 
\foii\       7321.47 & 
    3.47$\pm$   0.15 &     3.18$\pm$   0.14 & 
    3.30$\pm$   0.14 &     2.91$\pm$   0.13 & 
    2.75$\pm$   0.31 &     2.20$\pm$   0.25 & 
    3.25$\pm$   0.22 &     2.73$\pm$   0.18 \\ 
\foii\       7332.25 & 
    2.81$\pm$   0.15 &     2.58$\pm$   0.13 & 
    2.44$\pm$   0.14 &     2.15$\pm$   0.12 & 
    3.14$\pm$   0.32 &     2.51$\pm$   0.26 & 
    3.56$\pm$   0.23 &     2.99$\pm$   0.19 \\ 
\fsiii\      9071.10 & 
    12.7$\pm$    0.2 &     11.2$\pm$    0.2 & 
    11.0$\pm$    0.2 &      9.2$\pm$    0.1 & 
    16.1$\pm$    0.4 &     11.7$\pm$    0.3 & 
    11.7$\pm$    0.3 &      9.1$\pm$    0.2 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    431$\pm$      2} & 
\multicolumn{2}{c|}{    557$\pm$      2} & 
\multicolumn{2}{c|}{    247$\pm$      2} & 
\multicolumn{2}{c|}{    365$\pm$      2} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    533$\pm$      2} & 
\multicolumn{2}{c|}{    754$\pm$      3} & 
\multicolumn{2}{c|}{    424$\pm$      3} & 
\multicolumn{2}{c|}{    559$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.06$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.09$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined2_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~8} & \multicolumn{2}{c|}{\hii\ Reg~9 }& \multicolumn{2}{c|}{\hii\ Reg~10} & \multicolumn{2}{c|}{\hii\ Reg~11} \\
\hline\hline
\feiii\        4659.35 & 
    2.85$\pm$   0.92 &     2.91$\pm$   0.94 & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &       99$\pm$      1 \\ 
\foiii\        4960.29 & 
    39.0$\pm$    0.9 &     38.6$\pm$    0.9 & 
    97.4$\pm$    1.3 &     96.6$\pm$    1.3 & 
    20.3$\pm$    0.6 &     20.1$\pm$    0.6 & 
    45.5$\pm$    1.0 &     44.9$\pm$    1.0 \\ 
\foiii\       5008.24 & 
     114$\pm$      1 &      112$\pm$      1 & 
     287$\pm$      2 &      283$\pm$      2 & 
    62.5$\pm$    0.9 &     61.8$\pm$    0.8 & 
     139$\pm$      1 &      137$\pm$      1 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    6.73$\pm$   0.56 &     6.15$\pm$   0.51 & 
    10.4$\pm$    0.5 &      9.7$\pm$    0.5 & 
    7.65$\pm$   0.46 &     7.09$\pm$   0.43 & 
    9.97$\pm$   0.61 &     8.99$\pm$   0.55 \\ 
\foi\        6302.05 & 
    9.12$\pm$   0.63 &     8.09$\pm$   0.56 & 
    3.10$\pm$   0.53 &     2.80$\pm$   0.48 & 
    19.0$\pm$    0.5 &     17.1$\pm$    0.5 & 
    7.25$\pm$   0.69 &     6.32$\pm$   0.60 \\ 
\fsiii\       6313.80 & 
$<$   0.93  & $<$   0.82  & 
$<$   0.82  & $<$   0.74  & 
$<$   0.70  & $<$   0.64  & 
    2.74$\pm$   0.45 &     2.39$\pm$   0.39 \\ 
\foi\       6365.54 & 
    2.16$\pm$   0.42 &     1.91$\pm$   0.37 & 
    1.38$\pm$   0.36 &     1.24$\pm$   0.32 & 
    4.95$\pm$   0.34 &     4.45$\pm$   0.31 & 
    1.74$\pm$   0.43 &     1.51$\pm$   0.37 \\ 
\ha\       6564.61 & 
     320$\pm$      3 &      280$\pm$      3 & 
     315$\pm$      3 &      280$\pm$      2 & 
     314$\pm$      2 &      279$\pm$      2 & 
     327$\pm$      3 &      280$\pm$      3 \\ 
\fnii\        6585.20 & 
    16.3$\pm$    0.5 &     14.2$\pm$    0.4 & 
    9.12$\pm$   0.37 &     8.10$\pm$   0.33 & 
    18.2$\pm$    0.4 &     16.2$\pm$    0.3 & 
    13.4$\pm$    0.5 &     11.5$\pm$    0.4 \\ 
\hei\        6679.99 & 
    2.53$\pm$   0.37 &     2.20$\pm$   0.32 & 
    4.50$\pm$   0.33 &     3.97$\pm$   0.29 & 
    3.16$\pm$   0.29 &     2.80$\pm$   0.26 & 
    2.00$\pm$   0.41 &     1.69$\pm$   0.35 \\ 
\fsii\       6718.29 & 
    41.1$\pm$    0.6 &     35.5$\pm$    0.6 & 
    18.9$\pm$    0.4 &     16.7$\pm$    0.4 & 
    69.6$\pm$    0.7 &     61.5$\pm$    0.6 & 
    35.9$\pm$    0.6 &     30.3$\pm$    0.5 \\ 
\fsii\       6732.67 & 
    28.1$\pm$    0.5 &     24.3$\pm$    0.5 & 
    12.6$\pm$    0.4 &     11.1$\pm$    0.3 & 
    48.5$\pm$    0.5 &     42.8$\pm$    0.5 & 
    25.4$\pm$    0.5 &     21.4$\pm$    0.5 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    3.49$\pm$   0.38 &     2.95$\pm$   0.32 & 
    7.22$\pm$   0.34 &     6.24$\pm$   0.30 & 
    3.46$\pm$   0.31 &     2.99$\pm$   0.27 & 
    3.77$\pm$   0.43 &     3.10$\pm$   0.35 \\ 
\foii\       7321.47 & 
    3.52$\pm$   0.43 &     2.94$\pm$   0.36 & 
    2.78$\pm$   0.36 &     2.38$\pm$   0.31 & 
    3.28$\pm$   0.34 &     2.82$\pm$   0.29 & 
    3.86$\pm$   0.45 &     3.14$\pm$   0.37 \\ 
\foii\       7332.25 & 
    2.28$\pm$   0.44 &     1.90$\pm$   0.36 & 
$<$   0.49  & $<$   0.42  & 
    2.14$\pm$   0.34 &     1.83$\pm$   0.29 & 
    3.53$\pm$   0.47 &     2.87$\pm$   0.38 \\ 
\fsiii\      9071.10 & 
    11.2$\pm$    0.5 &      8.7$\pm$    0.4 & 
    15.1$\pm$    0.4 &     12.1$\pm$    0.3 & 
    7.29$\pm$   0.36 &     5.88$\pm$   0.29 & 
    12.5$\pm$    0.5 &      9.4$\pm$    0.4 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    143$\pm$      1} & 
\multicolumn{2}{c|}{    191$\pm$      1} & 
\multicolumn{2}{c|}{    234$\pm$      1} & 
\multicolumn{2}{c|}{    144$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    221$\pm$      2} & 
\multicolumn{2}{c|}{    278$\pm$      2} & 
\multicolumn{2}{c|}{    339$\pm$      2} & 
\multicolumn{2}{c|}{    237$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.11$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.11$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.15$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined3_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~12} & \multicolumn{2}{c|}{\hii\ Reg~13 }& \multicolumn{2}{c|}{\hii\ Reg~14} & \multicolumn{2}{c|}{\hii\ Reg~15} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      1 &       99$\pm$      1 \\ 
\foiii\        4960.29 & 
    73.3$\pm$    2.0 &     72.3$\pm$    2.0 & 
    60.0$\pm$    1.7 &     59.5$\pm$    1.7 & 
    37.3$\pm$    1.0 &     36.8$\pm$    1.0 & 
    41.3$\pm$    1.1 &     40.9$\pm$    1.1 \\ 
\foiii\       5008.24 & 
     219$\pm$      4 &      214$\pm$      4 & 
     175$\pm$      3 &      173$\pm$      3 & 
     103$\pm$      1 &      102$\pm$      1 & 
     130$\pm$      1 &      128$\pm$      1 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    13.1$\pm$    1.1 &     11.6$\pm$    1.0 & 
    8.38$\pm$   0.98 &     7.86$\pm$   0.92 & 
    8.63$\pm$   0.62 &     7.73$\pm$   0.55 & 
    10.8$\pm$    0.6 &      9.8$\pm$    0.6 \\ 
\foi\        6302.05 & 
    12.8$\pm$    1.2 &     10.9$\pm$    1.0 & 
    7.41$\pm$   1.06 &     6.81$\pm$   0.97 & 
    12.9$\pm$    0.7 &     11.1$\pm$    0.6 & 
    8.29$\pm$   0.76 &     7.28$\pm$   0.67 \\ 
\fsiii\       6313.80 & 
$<$   1.31  & $<$   1.12  & 
$<$   1.65  & $<$   1.52  & 
$<$   0.96  & $<$   0.83  & 
    2.55$\pm$   0.52 &     2.24$\pm$   0.46 \\ 
\foi\       6365.54 & 
--- & --- & 
    3.38$\pm$   0.70 &     3.10$\pm$   0.64 & 
    1.40$\pm$   0.46 &     1.20$\pm$   0.39 & 
--- & --- \\ 
\ha\       6564.61 & 
     337$\pm$      5 &      280$\pm$      4 & 
     308$\pm$      5 &      279$\pm$      4 & 
     330$\pm$      3 &      280$\pm$      3 & 
     324$\pm$      3 &      280$\pm$      3 \\ 
\fnii\        6585.20 & 
    24.2$\pm$    0.9 &     20.0$\pm$    0.7 & 
    12.1$\pm$    0.7 &     10.9$\pm$    0.6 & 
    15.1$\pm$    0.5 &     12.8$\pm$    0.4 & 
    17.9$\pm$    0.6 &     15.4$\pm$    0.5 \\ 
\hei\        6679.99 & 
    2.29$\pm$   0.70 &     1.89$\pm$   0.58 & 
--- & --- & 
    2.43$\pm$   0.40 &     2.04$\pm$   0.34 & 
    4.46$\pm$   0.45 &     3.82$\pm$   0.39 \\ 
\fsii\       6718.29 & 
    47.1$\pm$    1.1 &     38.6$\pm$    0.9 & 
    36.2$\pm$    0.9 &     32.7$\pm$    0.9 & 
    38.9$\pm$    0.6 &     32.5$\pm$    0.5 & 
    43.8$\pm$    0.7 &     37.4$\pm$    0.6 \\ 
\fsii\       6732.67 & 
    30.8$\pm$    0.9 &     25.3$\pm$    0.8 & 
    26.9$\pm$    0.8 &     24.3$\pm$    0.8 & 
    28.6$\pm$    0.5 &     23.9$\pm$    0.5 & 
    29.5$\pm$    0.6 &     25.1$\pm$    0.5 \\ 
\fneiii\        6870.16 & 
    4.48$\pm$   0.95 &     3.62$\pm$   0.77 & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\fariii\       7137.80 & 
    10.7$\pm$    0.7 &      8.5$\pm$    0.6 & 
    5.49$\pm$   0.68 &     4.87$\pm$   0.61 & 
    4.13$\pm$   0.42 &     3.36$\pm$   0.34 & 
    4.18$\pm$   0.45 &     3.48$\pm$   0.37 \\ 
\foii\       7321.47 & 
    6.02$\pm$   0.80 &     4.71$\pm$   0.63 & 
$<$   0.98  & $<$   0.87  & 
    2.27$\pm$   0.44 &     1.82$\pm$   0.35 & 
    2.80$\pm$   0.49 &     2.30$\pm$   0.41 \\ 
\foii\       7332.25 & 
    3.49$\pm$   0.80 &     2.73$\pm$   0.62 & 
    4.09$\pm$   0.76 &     3.60$\pm$   0.67 & 
    3.99$\pm$   0.47 &     3.20$\pm$   0.37 & 
    3.61$\pm$   0.49 &     2.97$\pm$   0.41 \\ 
\fsiii\      9071.10 & 
    16.9$\pm$    0.9 &     12.0$\pm$    0.6 & 
    14.8$\pm$    0.8 &     12.4$\pm$    0.7 & 
    10.4$\pm$    0.5 &      7.6$\pm$    0.4 & 
    11.1$\pm$    0.5 &      8.4$\pm$    0.4 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   73.7$\pm$    1.2} & 
\multicolumn{2}{c|}{   94.2$\pm$    1.5} & 
\multicolumn{2}{c|}{    172$\pm$      1} & 
\multicolumn{2}{c|}{    140$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    133$\pm$      2} & 
\multicolumn{2}{c|}{    127$\pm$      2} & 
\multicolumn{2}{c|}{    293$\pm$      3} & 
\multicolumn{2}{c|}{    224$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.18$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.09$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.14$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined4_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~16} & \multicolumn{2}{c|}{\hii\ Reg~17 }& \multicolumn{2}{c|}{\hii\ Reg~18} & \multicolumn{2}{c|}{\hii\ Reg~19} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      1 &       99$\pm$      1 \\ 
\foiii\        4960.29 & 
    38.7$\pm$    0.8 &     38.5$\pm$    0.8 & 
    48.3$\pm$    1.5 &     47.8$\pm$    1.5 & 
    56.0$\pm$    2.2 &     55.1$\pm$    2.2 & 
    9.97$\pm$   0.87 &     9.87$\pm$   0.86 \\ 
\foiii\       5008.24 & 
     112$\pm$      1 &      111$\pm$      1 & 
     132$\pm$      2 &      130$\pm$      2 & 
     155$\pm$      3 &      151$\pm$      3 & 
    37.0$\pm$    1.0 &     36.4$\pm$    1.0 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    8.69$\pm$   0.54 &     8.24$\pm$   0.52 & 
    8.87$\pm$   0.92 &     8.10$\pm$   0.84 & 
    13.8$\pm$    1.3 &     12.0$\pm$    1.2 & 
    6.99$\pm$   0.66 &     6.38$\pm$   0.60 \\ 
\foi\        6302.05 & 
    8.00$\pm$   0.66 &     7.45$\pm$   0.62 & 
    10.1$\pm$    1.1 &      9.0$\pm$    0.9 & 
    16.2$\pm$    1.6 &     13.5$\pm$    1.4 & 
    9.84$\pm$   0.75 &     8.72$\pm$   0.66 \\ 
\fsiii\       6313.80 & 
$<$   0.64  & $<$   0.60  & 
$<$   1.02  & $<$   0.90  & 
$<$   1.61  & $<$   1.34  & 
$<$   1.12  & $<$   0.99  \\ 
\foi\       6365.54 & 
    2.84$\pm$   0.42 &     2.64$\pm$   0.39 & 
    3.56$\pm$   0.65 &     3.14$\pm$   0.58 & 
    5.94$\pm$   1.07 &     4.92$\pm$   0.88 & 
    2.29$\pm$   0.51 &     2.02$\pm$   0.45 \\ 
\ha\       6564.61 & 
     303$\pm$      2 &      280$\pm$      2 & 
     320$\pm$      5 &      280$\pm$      4 & 
     344$\pm$      7 &      279$\pm$      5 & 
     321$\pm$      3 &      280$\pm$      3 \\ 
\fnii\        6585.20 & 
    13.9$\pm$    0.4 &     12.8$\pm$    0.4 & 
    9.35$\pm$   0.62 &     8.15$\pm$   0.54 & 
    21.6$\pm$    1.1 &     17.5$\pm$    0.9 & 
    17.2$\pm$    0.5 &     14.9$\pm$    0.5 \\ 
\hei\        6679.99 & 
    2.61$\pm$   0.36 &     2.40$\pm$   0.33 & 
    3.23$\pm$   0.57 &     2.80$\pm$   0.49 & 
    3.21$\pm$   0.95 &     2.58$\pm$   0.77 & 
    2.69$\pm$   0.45 &     2.33$\pm$   0.39 \\ 
\fsii\       6718.29 & 
    38.5$\pm$    0.6 &     35.3$\pm$    0.5 & 
    36.2$\pm$    0.9 &     31.3$\pm$    0.7 & 
    59.8$\pm$    1.6 &     47.9$\pm$    1.3 & 
    53.6$\pm$    0.8 &     46.3$\pm$    0.7 \\ 
\fsii\       6732.67 & 
    26.4$\pm$    0.5 &     24.2$\pm$    0.4 & 
    25.5$\pm$    0.7 &     22.0$\pm$    0.6 & 
    40.2$\pm$    1.3 &     32.1$\pm$    1.1 & 
    38.1$\pm$    0.7 &     32.9$\pm$    0.6 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
    5.32$\pm$   1.28 &     4.20$\pm$   1.01 & 
    1.76$\pm$   0.57 &     1.50$\pm$   0.49 \\ 
\fariii\       7137.80 & 
    4.44$\pm$   0.37 &     4.01$\pm$   0.34 & 
    4.70$\pm$   0.63 &     3.97$\pm$   0.53 & 
    3.39$\pm$   0.97 &     2.62$\pm$   0.75 & 
    1.83$\pm$   0.45 &     1.54$\pm$   0.38 \\ 
\foii\       7321.47 & 
    2.34$\pm$   0.40 &     2.10$\pm$   0.36 & 
    2.40$\pm$   0.67 &     2.00$\pm$   0.56 & 
$<$   2.05  & $<$   1.56  & 
    2.95$\pm$   0.52 &     2.46$\pm$   0.43 \\ 
\foii\       7332.25 & 
$<$   0.86  & $<$   0.78  & 
    4.25$\pm$   0.70 &     3.55$\pm$   0.58 & 
$<$   3.59  & $<$   2.73  & 
$<$   0.93  & $<$   0.78  \\ 
\fsiii\      9071.10 & 
    9.26$\pm$   0.44 &     7.98$\pm$   0.38 & 
    7.23$\pm$   0.67 &     5.62$\pm$   0.52 & 
    12.8$\pm$    1.1 &      8.7$\pm$    0.8 & 
    5.80$\pm$   0.53 &     4.49$\pm$   0.41 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    168$\pm$      1} & 
\multicolumn{2}{c|}{    107$\pm$      1} & 
\multicolumn{2}{c|}{   70.9$\pm$    1.4} & 
\multicolumn{2}{c|}{    151$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    217$\pm$      2} & 
\multicolumn{2}{c|}{    166$\pm$      2} & 
\multicolumn{2}{c|}{    137$\pm$      3} & 
\multicolumn{2}{c|}{    235$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.08$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.20$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.13$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined5_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~20} & \multicolumn{2}{c|}{\hii\ Reg~21 }& \multicolumn{2}{c|}{\hii\ Reg~22} & \multicolumn{2}{c|}{\hii\ Reg~23} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
    7.49$\pm$   2.02 &     7.55$\pm$   2.04 & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      2 &      100$\pm$      2 \\ 
\foiii\        4960.29 & 
    25.6$\pm$    1.0 &     25.4$\pm$    1.0 & 
    39.8$\pm$    1.8 &     39.1$\pm$    1.8 & 
    50.0$\pm$    2.2 &     49.7$\pm$    2.2 & 
    35.3$\pm$    1.5 &     34.9$\pm$    1.5 \\ 
\foiii\       5008.24 & 
    77.2$\pm$    1.4 &     76.2$\pm$    1.3 & 
     111$\pm$      2 &      108$\pm$      2 & 
     133$\pm$      3 &      132$\pm$      3 & 
     113$\pm$      2 &      112$\pm$      2 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    11.1$\pm$    0.7 &     10.3$\pm$    0.7 & 
    6.53$\pm$   1.18 &     5.60$\pm$   1.01 & 
    9.00$\pm$   1.31 &     8.49$\pm$   1.24 & 
    9.72$\pm$   0.97 &     8.93$\pm$   0.89 \\ 
\foi\        6302.05 & 
    10.5$\pm$    0.8 &      9.4$\pm$    0.7 & 
    29.1$\pm$    1.5 &     23.7$\pm$    1.2 & 
    11.2$\pm$    1.5 &     10.3$\pm$    1.4 & 
    9.89$\pm$   1.17 &     8.83$\pm$   1.04 \\ 
\fsiii\       6313.80 & 
$<$   0.79  & $<$   0.71  & 
$<$   1.28  & $<$   1.04  & 
$<$   2.21  & $<$   2.05  & 
$<$   1.70  & $<$   1.52  \\ 
\foi\       6365.54 & 
--- & --- & 
    9.87$\pm$   0.93 &     7.97$\pm$   0.75 & 
    3.17$\pm$   1.01 &     2.93$\pm$   0.93 & 
--- & --- \\ 
\ha\       6564.61 & 
     315$\pm$      3 &      280$\pm$      3 & 
     354$\pm$      6 &      280$\pm$      5 & 
     305$\pm$      6 &      280$\pm$      6 & 
     318$\pm$      5 &      280$\pm$      4 \\ 
\fnii\        6585.20 & 
    15.4$\pm$    0.6 &     13.6$\pm$    0.5 & 
    25.8$\pm$    1.0 &     20.3$\pm$    0.8 & 
    12.0$\pm$    1.0 &     11.0$\pm$    0.9 & 
    16.9$\pm$    0.8 &     14.8$\pm$    0.7 \\ 
\hei\        6679.99 & 
    1.88$\pm$   0.49 &     1.66$\pm$   0.43 & 
    3.67$\pm$   0.79 &     2.87$\pm$   0.62 & 
--- & --- & 
    3.31$\pm$   0.70 &     2.89$\pm$   0.61 \\ 
\fsii\       6718.29 & 
    48.1$\pm$    0.8 &     42.2$\pm$    0.7 & 
    87.6$\pm$    1.9 &     68.2$\pm$    1.5 & 
    31.7$\pm$    1.2 &     28.8$\pm$    1.1 & 
    40.3$\pm$    1.0 &     35.1$\pm$    0.9 \\ 
\fsii\       6732.67 & 
    33.4$\pm$    0.7 &     29.4$\pm$    0.6 & 
    61.8$\pm$    1.5 &     48.0$\pm$    1.2 & 
    24.8$\pm$    1.1 &     22.6$\pm$    1.0 & 
    29.0$\pm$    0.9 &     25.2$\pm$    0.8 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
    2.73$\pm$   0.89 &     2.36$\pm$   0.77 \\ 
\fariii\       7137.80 & 
    4.01$\pm$   0.50 &     3.45$\pm$   0.43 & 
    3.69$\pm$   0.82 &     2.75$\pm$   0.61 & 
    6.38$\pm$   0.89 &     5.72$\pm$   0.80 & 
    5.25$\pm$   0.67 &     4.47$\pm$   0.57 \\ 
\foii\       7321.47 & 
    3.70$\pm$   0.53 &     3.16$\pm$   0.45 & 
    4.68$\pm$   0.90 &     3.43$\pm$   0.66 & 
$<$   1.97  & $<$   1.75  & 
    3.79$\pm$   0.72 &     3.20$\pm$   0.61 \\ 
\foii\       7332.25 & 
    4.29$\pm$   0.54 &     3.65$\pm$   0.46 & 
$<$   1.88  & $<$   1.38  & 
$<$   1.56  & $<$   1.38  & 
$<$   1.53  & $<$   1.29  \\ 
\fsiii\      9071.10 & 
    8.33$\pm$   0.55 &     6.66$\pm$   0.44 & 
    11.3$\pm$    0.9 &      7.3$\pm$    0.6 & 
    12.7$\pm$    1.0 &     10.8$\pm$    0.9 & 
    12.7$\pm$    0.8 &     10.0$\pm$    0.6 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    147$\pm$      1} & 
\multicolumn{2}{c|}{   90.4$\pm$    1.7} & 
\multicolumn{2}{c|}{   66.3$\pm$    1.4} & 
\multicolumn{2}{c|}{   91.9$\pm$    1.4} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    216$\pm$      2} & 
\multicolumn{2}{c|}{    191$\pm$      4} & 
\multicolumn{2}{c|}{   87.9$\pm$    1.9} & 
\multicolumn{2}{c|}{    138$\pm$      2} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.12$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.23$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.08$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.12$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined6_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. }& \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~.} \\
 & \multicolumn{2}{c|}{\hii\ Reg~24} & \multicolumn{2}{c|}{\hii\ Reg~25 }& \multicolumn{2}{c|}{\hii\ Reg~26} & \multicolumn{2}{c|}{\hii\ Reg~27} \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
    7.23$\pm$   2.29 &     7.48$\pm$   2.37 & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      2 &      100$\pm$      2 & 
     100$\pm$      3 &      100$\pm$      3 & 
     100$\pm$      1 &      100$\pm$      1 & 
     100$\pm$      2 &      100$\pm$      2 \\ 
\foiii\        4960.29 & 
    73.2$\pm$    2.0 &     71.9$\pm$    2.0 & 
    32.3$\pm$    2.0 &     31.8$\pm$    2.0 & 
     110$\pm$      2 &      109$\pm$      2 & 
    34.2$\pm$    1.4 &     33.7$\pm$    1.4 \\ 
\foiii\       5008.24 & 
     227$\pm$      4 &      221$\pm$      4 & 
    73.5$\pm$    2.5 &     71.9$\pm$    2.5 & 
     335$\pm$      5 &      330$\pm$      4 & 
     108$\pm$      2 &      106$\pm$      2 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    10.4$\pm$    1.1 &      8.9$\pm$    0.9 & 
    5.17$\pm$   1.30 &     4.52$\pm$   1.14 & 
    11.1$\pm$    0.9 &     10.0$\pm$    0.8 & 
    9.45$\pm$   1.00 &     8.32$\pm$   0.88 \\ 
\foi\        6302.05 & 
    8.22$\pm$   1.22 &     6.68$\pm$   0.99 & 
    20.3$\pm$    1.7 &     16.9$\pm$    1.4 & 
    12.8$\pm$    1.1 &     11.1$\pm$    0.9 & 
    16.1$\pm$    1.1 &     13.6$\pm$    0.9 \\ 
\fsiii\       6313.80 & 
$<$   1.22  & $<$   0.99  & 
$<$   2.28  & $<$   1.91  & 
    3.84$\pm$   0.70 &     3.32$\pm$   0.61 & 
$<$   1.10  & $<$   0.92  \\ 
\foi\       6365.54 & 
--- & --- & 
    4.72$\pm$   1.00 &     3.92$\pm$   0.83 & 
    3.22$\pm$   0.69 &     2.78$\pm$   0.59 & 
    5.54$\pm$   0.71 &     4.65$\pm$   0.60 \\ 
\ha\       6564.61 & 
     354$\pm$      6 &      280$\pm$      5 & 
     343$\pm$      7 &      280$\pm$      6 & 
     329$\pm$      4 &      280$\pm$      4 & 
     339$\pm$      5 &      279$\pm$      4 \\ 
\fnii\        6585.20 & 
    17.7$\pm$    0.8 &     14.0$\pm$    0.7 & 
    14.3$\pm$    1.0 &     11.7$\pm$    0.8 & 
    16.1$\pm$    0.7 &     13.7$\pm$    0.6 & 
    24.4$\pm$    0.8 &     20.1$\pm$    0.7 \\ 
\hei\        6679.99 & 
    3.49$\pm$   0.71 &     2.72$\pm$   0.56 & 
--- & --- & 
    1.92$\pm$   0.60 &     1.62$\pm$   0.51 & 
    4.33$\pm$   0.65 &     3.53$\pm$   0.53 \\ 
\fsii\       6718.29 & 
    40.3$\pm$    1.1 &     31.3$\pm$    0.8 & 
    59.9$\pm$    1.6 &     48.2$\pm$    1.3 & 
    42.8$\pm$    0.9 &     36.0$\pm$    0.8 & 
    64.7$\pm$    1.3 &     52.6$\pm$    1.1 \\ 
\fsii\       6732.67 & 
    27.8$\pm$    0.9 &     21.6$\pm$    0.7 & 
    41.0$\pm$    1.3 &     32.9$\pm$    1.1 & 
    33.6$\pm$    0.8 &     28.2$\pm$    0.7 & 
    45.0$\pm$    1.0 &     36.5$\pm$    0.8 \\ 
\fneiii\        6870.16 & 
--- & --- & 
--- & --- & 
--- & --- & 
    3.74$\pm$   0.91 &     3.00$\pm$   0.73 \\ 
\fariii\       7137.80 & 
    6.80$\pm$   0.72 &     5.07$\pm$   0.54 & 
--- & --- & 
    7.91$\pm$   0.62 &     6.46$\pm$   0.50 & 
    7.23$\pm$   0.70 &     5.69$\pm$   0.55 \\ 
\foii\       7321.47 & 
    3.31$\pm$   0.75 &     2.43$\pm$   0.55 & 
    5.77$\pm$   1.02 &     4.40$\pm$   0.78 & 
    3.95$\pm$   0.63 &     3.19$\pm$   0.51 & 
$<$   1.51  & $<$   1.17  \\ 
\foii\       7332.25 & 
$<$   1.13  & $<$   0.83  & 
    4.66$\pm$   1.00 &     3.55$\pm$   0.76 & 
    3.87$\pm$   0.64 &     3.12$\pm$   0.52 & 
$<$   2.70  & $<$   2.09  \\ 
\fsiii\      9071.10 & 
    16.3$\pm$    0.9 &     10.5$\pm$    0.6 & 
    7.15$\pm$   1.03 &     4.89$\pm$   0.71 & 
    15.3$\pm$    0.7 &     11.3$\pm$    0.5 & 
    13.9$\pm$    0.8 &      9.7$\pm$    0.5 \\ 
 & & & & & & & & \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   89.8$\pm$    1.6} & 
\multicolumn{2}{c|}{   71.5$\pm$    1.5} & 
\multicolumn{2}{c|}{    109$\pm$      1} & 
\multicolumn{2}{c|}{    106$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{    190$\pm$      4} & 
\multicolumn{2}{c|}{    137$\pm$      3} & 
\multicolumn{2}{c|}{    183$\pm$      2} & 
\multicolumn{2}{c|}{    196$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.23$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.20$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.19$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/All_fluxes_combined7_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|l|cc|cc|}
\hline
 & \multicolumn{2}{c|}{\hii\ Reg~.} & \multicolumn{2}{c|}{\hii\ Reg~. } \\
 & \multicolumn{2}{c|}{\hii\ Reg~28} & \multicolumn{2}{c|}{\hii\ Reg~29 } \\
\hline\hline
\feiii\        4659.35 & 
--- & --- & 
--- & --- \\ 
\heii\        4687.02 & 
--- & --- & 
--- & --- \\ 
\ariv\        4741.49 & 
--- & --- & 
--- & --- \\ 
\hb\        4862.72 & 
     100$\pm$      3 &      100$\pm$      3 & 
     100$\pm$      2 &      100$\pm$      2 \\ 
\foiii\        4960.29 & 
    31.2$\pm$    2.4 &     30.8$\pm$    2.3 & 
    20.5$\pm$    1.3 &     20.2$\pm$    1.2 \\ 
\foiii\       5008.24 & 
     103$\pm$      3 &      101$\pm$      3 & 
    58.4$\pm$    1.5 &     57.2$\pm$    1.5 \\ 
\fnii\       5756.24 & 
--- & --- & 
--- & --- \\ 
\hei\        5877.59 & 
    10.1$\pm$    1.6 &      9.0$\pm$    1.4 & 
    7.60$\pm$   0.91 &     6.66$\pm$   0.80 \\ 
\foi\        6302.05 & 
    13.1$\pm$    2.0 &     11.4$\pm$    1.7 & 
    12.4$\pm$    1.0 &     10.4$\pm$    0.9 \\ 
\fsiii\       6313.80 & 
$<$   1.97  & $<$   1.70  & 
$<$   1.59  & $<$   1.33  \\ 
\foi\       6365.54 & 
--- & --- & 
--- & --- \\ 
\ha\       6564.61 & 
     330$\pm$      8 &      280$\pm$      7 & 
     342$\pm$      5 &      279$\pm$      4 \\ 
\fnii\        6585.20 & 
    12.7$\pm$    1.3 &     10.8$\pm$    1.1 & 
    20.5$\pm$    0.7 &     16.8$\pm$    0.6 \\ 
\hei\        6679.99 & 
--- & --- & 
    3.10$\pm$   0.61 &     2.51$\pm$   0.50 \\ 
\fsii\       6718.29 & 
    26.5$\pm$    1.4 &     22.2$\pm$    1.2 & 
    57.3$\pm$    1.1 &     46.3$\pm$    0.9 \\ 
\fsii\       6732.67 & 
    16.9$\pm$    1.2 &     14.1$\pm$    1.0 & 
    39.3$\pm$    0.9 &     31.7$\pm$    0.7 \\ 
\fneiii\        6870.16 & 
    5.16$\pm$   1.46 &     4.28$\pm$   1.21 & 
--- & --- \\ 
\fariii\       7137.80 & 
    3.89$\pm$   1.06 &     3.17$\pm$   0.87 & 
    2.67$\pm$   0.63 &     2.08$\pm$   0.49 \\ 
\foii\       7321.47 & 
$<$   2.36  & $<$   1.90  & 
$<$   0.98  & $<$   0.75  \\ 
\foii\       7332.25 & 
    8.10$\pm$   1.18 &     6.50$\pm$   0.95 & 
$<$   1.10  & $<$   0.84  \\ 
\fsiii\      9071.10 & 
    13.8$\pm$    1.4 &     10.2$\pm$    1.0 & 
    11.0$\pm$    0.7 &      7.6$\pm$    0.5 \\ 
 & & & &  \\
F(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   48.9$\pm$    1.2} & 
\multicolumn{2}{c|}{    109$\pm$      1} \\ 
I(\hb) $\times 10^{-18}$ erg s$^{-1}$ cm$^{-2}$ &
\multicolumn{2}{c|}{   82.8$\pm$    2.3} & 
\multicolumn{2}{c|}{    207$\pm$      3} \\ 
E(B-V) &
\multicolumn{2}{c|}{ 0.16$\pm$ 0.00} & 
\multicolumn{2}{c|}{ 0.19$\pm$ 0.00} \\ 
\hline
\hline
\end{tabular}
\label{tab:fluxes_all}
\end{footnotesize}
\end{center}


==> MUSE_ JKB18/all_abund_bin7v2.tex <==
\begin{center}
\begin{footnotesize}
\begin{tabular}{|c|ccccccccc|}
\hline
\hii\ Reg ID & \eld(\fsii ) & \elt(\fsiii)  & \elt(\foii) & \op/\hp & \opp /\hp  & 12+log(O/H) & log(N/O) & 12+log(N/H) & [O/H] \\
 & (cm$^{-3}$)  & (K) & (K) & ($\times10^{-5}$) & ($\times10^{-5}$) & Z[Direct] & &  & Z[O3N2] \\ 
\hline
0& 
13$\pm$7.8 & 
15300$\pm$490&
20100$\pm$586&
   0.70$\pm$   0.08&
   2.20$\pm$   0.18&
   7.46$\pm$   0.03&
  -1.15$\pm$   0.02&
   6.31$\pm$   0.02&
8.33$\pm$0.05 \\
1& 
41$\pm$9.5 & 
14200$\pm$619&
18600$\pm$740&
   1.15$\pm$   0.18&
   2.10$\pm$   0.24&
   7.51$\pm$   0.04&
  -1.07$\pm$   0.03&
   6.44$\pm$   0.03&
8.43$\pm$0.04 \\
2& 
22$\pm$11 & 
12800$\pm$605&
16600$\pm$723&
   1.26$\pm$   0.24&
   4.78$\pm$   0.65&
   7.78$\pm$   0.05&
  -1.28$\pm$   0.04&
   6.50$\pm$   0.04&
8.27$\pm$0.05 \\
3& 
28$\pm$13 & 
12400$\pm$668&
15900$\pm$798&
   1.02$\pm$   0.25&
   5.65$\pm$   0.91&
   7.82$\pm$   0.06&
  -1.27$\pm$   0.04&
   6.56$\pm$   0.04&
8.22$\pm$0.04 \\
4& 
36$\pm$14 & 
14400$\pm$947&
18800$\pm$1130&
   1.03$\pm$   0.24&
   2.59$\pm$   0.46&
   7.56$\pm$   0.06&
  -1.28$\pm$   0.04&
   6.28$\pm$   0.04&
8.34$\pm$0.06 \\
5& 
13$\pm$8.8 & 
11300$\pm$823&
14400$\pm$984&
   2.69$\pm$   0.88&
   4.32$\pm$   1.02&
   7.85$\pm$   0.08&
  -1.43$\pm$   0.06&
   6.41$\pm$   0.06&
8.36$\pm$0.06 \\
6& 
36$\pm$19 & 
15100$\pm$1500&
19800$\pm$1790&
   0.70$\pm$   0.25&
   3.04$\pm$   0.79&
   7.57$\pm$   0.10&
  -1.01$\pm$   0.07&
   6.56$\pm$   0.07&
8.34$\pm$0.05 \\
7& 
18$\pm$12 & 
16600$\pm$1480&
22000$\pm$1770&
   0.61$\pm$   0.17&
   1.51$\pm$   0.32&
   7.33$\pm$   0.08&
  -1.12$\pm$   0.05&
   6.21$\pm$   0.05&
8.37$\pm$0.04 \\
8& 
12$\pm$12 & 
$<$11700&
$<$15000&
$>$   2.14&
$>$   2.44&
$>$   7.66&
--&
$>$   6.39&
8.47$\pm$0.05 \\
9& 
18$^{+18}_{-18}$ & 
$<$9580&
$<$12000&
$>$   3.64&
$>$  11.97&
$>$   8.19&
--&
$>$   6.66&
8.29$\pm$0.07 \\
10& 
17$\pm$10. & 
$<$12500&
$<$16200&
$>$   1.49&
$>$   1.08&
$>$   7.41&
--&
$>$   6.29&
8.53$\pm$0.03 \\
11& 
41$\pm$25 & 
16600$\pm$1480$^\star$&
22000$\pm$1770&
   0.63$\pm$   0.20&
   1.16$\pm$   0.25&
   7.25$\pm$   0.08&
  -1.12$\pm$   0.06&
   6.13$\pm$   0.06&
8.41$\pm$0.04 \\
12& 
1.7$^{+4.3}_{-1.7}$ & 
$<$11600&
$<$14900&
$>$   3.47&
$>$   4.78&
$>$   7.92&
--&
$>$   6.59&
8.44$\pm$0.06 \\
13& 
100$\pm$44 & 
$<$13400&
$<$17500&
$>$   0.99&
$>$   2.53&
$>$   7.55&
--&
$>$   6.38&
8.41$\pm$0.07 \\
14& 
86$\pm$27 & 
$<$12600&
$<$16200&
$>$   1.50&
$>$   1.82&
$>$   7.52&
--&
$>$   6.29&
8.45$\pm$0.06 \\
15& 
9.5$^{+10.}_{-9.5}$ & 
15300$\pm$514$^\star$&
20100$\pm$614&
   0.75$\pm$   0.19&
   1.31$\pm$   0.12&
   7.31$\pm$   0.05&
  -1.01$\pm$   0.03&
   6.31$\pm$   0.03&
8.43$\pm$0.05 \\
16& 
14$\pm$13 & 
$<$10500&
$<$13300&
$>$   2.21&
$>$   3.42&
$>$   7.75&
--&
$>$   6.53&
8.45$\pm$0.04 \\
17& 
40$\pm$29 & 
$<$15800&
$<$20900&
$>$   0.69&
$>$   1.27&
$>$   7.29&
--&
$>$   6.02&
8.40$\pm$0.08 \\
18& 
20$\pm$19 & 
$<$15400&
$<$20300&
$>$   0.59&
$>$   1.57&
$>$   7.34&
--&
$>$   6.48&
8.45$\pm$0.05 \\
19& 
43$\pm$21 & 
$<$19900&
$<$26700&
$>$   0.19&
$>$   0.20&
$>$   6.59&
--&
$>$   5.98&
8.56$\pm$0.04 \\
20& 
24$\pm$19 & 
$<$12400&
$<$16000&
$>$   2.25&
$>$   1.38&
$>$   7.56&
--&
$>$   6.19&
8.50$\pm$0.04 \\
21& 
33$\pm$20 & 
$<$14700&
$<$19300&
$>$   0.79&
$>$   1.27&
$>$   7.31&
--&
$>$   6.44&
8.49$\pm$0.04 \\
22& 
180$\pm$71 & 
$<$17800&
$<$23700&
$>$   0.24&
$>$   0.99&
$>$   7.09&
--&
$>$   6.33&
8.43$\pm$0.05 \\
23& 
59$\pm$36 & 
$<$15300&
$<$20100&
$>$   0.62&
$>$   1.14&
$>$   7.25&
--&
$>$   6.31&
8.47$\pm$0.04 \\
24& 
32$\pm$27 & 
$<$11700&
$<$15000&
$>$   1.43&
$>$   4.79&
$>$   7.79&
--&
$>$   6.69&
8.36$\pm$0.04 \\
25& 
23$\pm$21 & 
$<$25000&
$<$33900&
$>$   0.26&
$>$   0.29&
$>$   6.74&
--&
$>$   5.76&
8.49$\pm$0.04 \\
26& 
180$\pm$39 & 
15100$\pm$1540$^\star$&
19900$\pm$1840&
   0.83$\pm$   0.34&
   3.50$\pm$   0.94&
   7.64$\pm$   0.10&
  -1.09$\pm$   0.07&
   6.54$\pm$   0.07&
8.35$\pm$0.07 \\
27& 
23$\pm$18 & 
$<$11800&
$<$15100&
$>$   1.40&
$>$   2.24&
$>$   7.56&
--&
$>$   6.62&
8.50$\pm$0.04 \\
28& 
48$\pm$44 & 
$<$16300&
$<$21500&
$>$   0.93&
$>$   0.88&
$>$   7.26&
--&
$>$   5.96&
8.42$\pm$0.08 \\
29& 
17$\pm$16 & 
$<$16800&
$<$22200&
$>$   0.16&
$>$   0.48&
$>$   6.81&
--&
$>$   6.43&
8.29$\pm$0.07 \\
\hline
\end{tabular}
\label{tab:abunds}
\end{footnotesize}
\end{center}

